Generative Models for Synthetic Urban Mobility Data: A Systematic Literature Review

Although highly valuable for a variety of applications, urban mobility data is rarely made openly available as it contains sensitive personal information. Synthetic data aims to solve this issue by generating artificial data that resembles an original dataset in structural and statistical characteristics, but omits sensitive information. For mobility data, a large number of corresponding models have been proposed in the last decade. This systematic review provides a structured comparative overview of the current state of this heterogeneous, active field of research. A special focus is put on the applicability of the reviewed models in practice.

==> figures/tikz_tex/taxonomy.tex <==
\begin{tikzpicture}

\tikzstyle{system}=[draw=black, rounded corners, font=\scriptsize,   inner sep=4.7pt, align=center, fill=white]
\tikzstyle{dots}=[draw=black, rounded corners, font=\scriptsize,   inner sep=7.3pt, align=center, fill=white]
\tikzstyle{text}=[font=\scriptsize]
\tikzstyle{section}=[fill=gray, opacity=0.1, rounded corners]

%background
\draw[section] grid(0,0) rectangle (14,0.8);
\draw[section] grid(0,1.2) rectangle (14,2);
\draw[section] grid(0,2.4) rectangle (14,3.2);

\node[text] (a) at (2.49, 0.4) {Similarity measures:};
\node[text] (b) at (2.45, 1.6) {Operationalized by:};
\node[text] (b) at (2.8, 2.8) {Mobility characteristics:};

%symbols
\node (ruler) at (0.44,0.4) {\includegraphics[width=12pt]{figures/ruler.png}};
\node (gear) at (0.5,1.6) {\includegraphics[width=14pt]{figures/gear.png}};
\node (thought) at (0.49,2.8) {\includegraphics[width=14pt]{figures/thought.png}};

%nodes
\node[system] (spatial) at (9, 2.8) {Spatial distribution};
\node[dots] (dots1) at (11.5, 2.8) {...};
\node[dots] (dots1.5) at (13, 2.8) {...};
\node[system] (location) at (6.5, 1.6) {location popularity ranking};
\node[system] (visits) at (10, 1.6) {visits per location};
\node[dots] (dots2) at (12.5, 1.6) {...};
\node[system] (kendall) at (6.5, 0.4) {Kendall-tau coefficient};
\node[system] (kld) at (9, 0.4) {KLD};
\node[system] (jsd) at (10, 0.4) {JSD};
\node[dots] (dots3) at (11, 0.4) {...};


%node connections
\draw[black] (spatial) -> (visits);
\draw[black] (spatial) -> (location);
\draw[black] (spatial) -> (dots2);

\draw[black] (location) -> (kendall);
\draw[black] (visits) -> (kld);
\draw[black] (visits) -> (jsd);
\draw[black] (visits) -> (dots3);

%big arrows
\draw[black, -latex, line width=0.5mm] (0.5,2.4) -> (0.5,2);
\draw[black, -latex, line width=0.5mm] (0.5,1.2) -> (0.5,0.8);

%\draw[gray,very thin,opacity=0.2] grid(15,5)foreach~in{0,1,...,4}{(1*~,-.1)node{\pgfmathprintnumber{~}}(-.1,1*~)node{\pgfmathprintnumber{~}}};
\end{tikzpicture}


==> figures/tikz_tex/tree.tex <==

\tikzset{level 1/.style={level distance=1cm, sibling distance=6cm,font=\scriptsize},
       level 2/.style={level distance=1cm, sibling distance=3.5cm,font=\scriptsize}}
       
\begin{tikzpicture}[sibling distance=13em, 
  every node/.style = {shape=rectangle, rounded corners,
    draw, align=center, font=\small}]
  \node {Utility evaluation measures}
    child { node {Downstream tasks} }
    child { node {Similarity measures} 
      child { node {Per-instance similarity} }
      child { node {Visual comparison} }
      child { node {Statistical similarity} } };
\end{tikzpicture}

